RLIF: Interactive Imitation Learning as Reinforcement Learning

Although reinforcement learning methods offer a powerful framework for automatic skill acquisition, for practical learning-based control problems in domains such as robotics, imitation learning often provides a more convenient and accessible alternative. In particular, an interactive imitation learning method such as DAgger, which queries a near-optimal expert to intervene online to collect correction data for addressing the distributional shift challenges that afflict na\"ive behavioral cloning, can enjoy good performance both in theory and practice without requiring manually specified reward functions and other components of full reinforcement learning methods. In this paper, we explore how off-policy reinforcement learning can enable improved performance under assumptions that are similar but potentially even more practical than those of interactive imitation learning. Our proposed method uses reinforcement learning with user intervention signals themselves as rewards. This relaxes the assumption that intervening experts in interactive imitation learning should be near-optimal and enables the algorithm to learn behaviors that improve over the potential suboptimal human expert. We also provide a unified framework to analyze our RL method and DAgger; for which we present the asymptotic analysis of the suboptimal gap for both methods as well as the non-asymptotic sample complexity bound of our method. We then evaluate our method on challenging high-dimensional continuous control simulation benchmarks as well as real-world robotic vision-based manipulation tasks. The results show that it strongly outperforms DAgger-like approaches across the different tasks, especially when the intervening experts are suboptimal. Code and videos can be found on the project website: https://rlif-page.github.io

==> sections/marked_changes/experiment.tex <==
\section{Experiments}\label{sec:experiments}

Since our method operates under standard interactive imitation learning assumptions, our experiments aim to compare RLIF to DAgger under different types of suboptimal experts and intervention modes. We seek to answer the following questions: (1) Are the intervention rewards sufficient signal for RL to learn effective policies? (2) How well does our method perform compared to DAgger, especially with suboptimal experts? (3) What are the implications of different intervention strategies on empirical performance?


\subsection{Intervention Strategies}
\label{subsec:intervention_mode}

\begin{wrapfigure}{rb}{0.4\textwidth}
    \vspace{-3em}
    \centering
     \includegraphics[width=0.4\textwidth]{figs/Setup.png} 
    \vspace{-1.5em}

    
    % \hspace{-0.25cm}\begin{minipage}[t]{0.07\textwidth}
    %     {\scriptsize a)Left camera}
    % \end{minipage}
    % % \hspace{10pt}
    %  \begin{minipage}[t]{0.07\textwidth}
    %     {\scriptsize b)Right camera}
    % \end{minipage}
    % \begin{minipage}[t]{0.07\textwidth}
    %     \centering
    %     {\scriptsize c)Space Mouse}
    % \end{minipage}
    \caption{\changed{Human supervises policy training and provides intervention with a Space Mouse device.}}
    \label{fig:human}
    % \vspace{-1em}
\end{wrapfigure}



In order to learn from interventions, we need the intervening experts to convey useful information about the task through their decision about \emph{when} to intervene. Since real human experts are likely to be imperfect in making this decision, we study a variety of intervention strategies in simulation empirically to validate the stability of our method with respect to this assumption. The baseline strategy, which we call \textbf{Random Intervention}, simply intervenes uniformly at random, with equal probability at every step. The more intelligent model, \textbf{Value-Based Intervention}, strategy assumes the expert intervenes with probability $\beta$ when there is a gap $\delta$ between actions from the expert and agent w.r.t. a reference value function $Q^{\piref}$. This model aims to capture an uncertain and stochastic expert, who might have a particular policy $\piexp$ that they use to choose actions (which could be highly suboptimal), and a \emph{separate} value function $Q^{\piref}$ with its corresponding policy $\piref$ that they use to determine if the robot is doing well or not, which they use to determine when to intervene. Note that $\piref$ might be much better than $\piexp$ -- for example, a human expert might correctly determine the robot is choosing poor actions for the task, even if their own policy $\piexp$ is not good enough to perform the task either.
%: independent of how optimal their actual policies are, \emph{how good do they think they are?} $Q^{\piref}$ is the reference model experts calibrate their decisions; where $\piref$ can be better or worse than $\piexp$, implying experts can make decisions when to intervene regardless of the suboptimality of their own policies.
$\delta$ represents the confidence level of the intervening expert: the smaller $\delta$ is, the more willing they are to intervene on even slightly suboptimal robot actions.
%This is more realistic because humans can never be always accurate about all the decisions they make, having a varying reference model $Q^{\piref}$ will reasonably capture that reality; thus allowing us to study the performance of our algorithm under different intervention modes.
We formalize this model in Eq.~\ref{eq:soft-rational-intervention}; in practice, we choose a value for $\beta$ close to 1 such as 0.95.
\begin{equation}
\label{eq:soft-rational-intervention}
\bb P(\textit{Intervention} | s) = 
  \begin{cases}
    \beta, & \text{if} \; Q^{\piref}(s, \piexp    (s)) > Q^{\piref}(s, \pi(s)) + \delta\\
    1 - \beta, & \text{otherwise}.
  \end{cases}
\end{equation}
This model may not be fully representative of real human behavior, so we also evaluate our method with real human interventions, where an expert user provides intervention feedback to a real-world robotic system performing a peg insertion task, shown in Figure~\ref{fig:human}. We discuss this further in Sec.~\ref{subsec:robot_task}.

In Appendix~\ref{sec:appendix_gridworld}, we also present a didactic experiment with the Grid World environment where we use value iteration as the underlying RL algorithm, to verify that RLIF does indeed converge to the optimal policy under idealized assumptions when we remove approximation and sampling error of the RL method from consideration.

\subsection{Performance on Continuous Control Benchmark Tasks}
Next, we evaluate RLIF in comparison with various interactive imitation learning methods on several high-dimensional continuous control benchmark tasks. These experiments vary both the optimality of the expert's policies and the expert's intervention strategy.

\begin{wrapfigure}{r}{0.55\textwidth}
    \centering
     \includegraphics[width=0.55\textwidth]{figs/rlif_train.png}
    % \vspace{-0.5em}
    \caption{Average success rate and intervention rate for the Adroit-Pen task during training, as the agent improves, the intervention decreases.}
    \label{fig:rlif_train}
\end{wrapfigure}

\paragraph{Simulation experiment setup.} 
We use Gym locomotion and Adroit dexterous manipulation tasks in these experiments, based on the D4RL environments~\citep{fu2020d4rl}. The Adroit environments require controlling a 24-DoF robotic hand to perform tasks such as opening a door or rotating a pen to randomly sampled goal locations. The Gym locomotion task (walker) requires controlling a planar 2-legged robot to walk forward. Both domains require continuous control at relatively high frequencies, where approximation errors and distributional shift can accumulate quickly for na\"{i}ve imitation learning methods. 
Note that although these benchmarks are often used to evaluate the performance of RL algorithms, we do not assume access to any reward function beyond the signal obtained from the expert's interventions, and therefore our main point of comparison are DAgger variants, rather than prior RL algorithms. 

\begin{figure*}[t!]

    \centering
    \vspace{-1cm}
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}[t]{ccccc}
     \includegraphics[width=.16\textwidth]{figs/locomotion.png} 
     & \includegraphics[width=.183\textwidth]{figs/pen.png}
     & \includegraphics[width=.16\textwidth]{figs/hopper.png}
     & \includegraphics[width=.1715\textwidth]{figs/robot.png}
     & \includegraphics[width=.173\textwidth]{figs/cloth.png}
     \\
    \end{tabular}
    
    
    \caption{\changed{\textbf{Tasks in our experimental evaluation}: Benchmark tasks Walker2d, Pen, and Hopper and two vision-based contact-rich manipulation tasks on a real robot. The benchmark tasks require handling complex high-dimensional dynamics and underactuation. The robotic insertion task requires additionally addressing complex inputs such as images, non-differentiable dynamics such as contact, and all sensor noise associated with real-world robotic settings.}}
    \label{fig:d4rl}
    \vspace{-0.3cm}
\end{figure*}





\begin{table*}[t]
\scriptsize{
\begin{center}
\vspace{-0.9cm}
\scalebox{0.9}{
% \begin{adjustwidth}{-1cm}{0cm}{-1cm}{-1cm}{-1cm}{-1cm}{-1cm}{-1cm}
\begin{tabular}
{p{1.5cm} p{0.7cm}|| p{1.2cm} p{1.3cm}|p{1.3cm} p{1.3cm} p{1.0cm} p{1.4cm} |p{1.2cm}}

Domain & Expert Level & RLIF with Value Based Intervention & RLIF with Random Intervention & HG-DAgger & HG-DAgger with 85\% Random Intervention & DAgger & DAgger with 85\% Random Intervention & BC \\ \hline
\texttt{adroit-pen} &\texttt{$\sim$90\%}  & \textbf{88.47$\pm$3.06} &  42.87$\pm$12.86 & 73.47$\pm$6.19 & 74.27$\pm$5.79 & 78.13$\pm$3.24 & 79.07$\pm$9 &  \\
 &\texttt{$\sim$40\%}  & \textbf{80.87$\pm$6.01} & 34.13$\pm$10.32 &  60$\pm$3.58 & 29.33$\pm$6.56 & 35.73$\pm$7.49 & 38.67$\pm$2.06 & 54.13$\pm$14.24 \\
 & \texttt{$\sim$10\%} &  \textbf{64.04$\pm$17.59} & 28.33$\pm$4.43 & 28.53$\pm$7.66 &  9.47$\pm$4.09 & 8.93$\pm$1.43 & 12.8$\pm$6.25 & \\ \hline 
 & average & \textbf{77.79$\pm$8.89}  & 35.11$\pm$9.20 & 54$\pm$5.81 & 37.69$\pm$5.48 & 40.93$\pm$4.05 & 43.51$\pm$5.77 & 54.13$\pm$14.24 \\ \hline 
\texttt{locomotion-}  &\texttt{$\sim$110\%} & 108.99$\pm$5.28 & 106.51$\pm$0.47 & 53.55$\pm$9.76 & \textbf{112.7$\pm$2.51} & 57.94$\pm$8.69 & 76.13$\pm$3.27 &  \\
 \texttt{walker2d} &\texttt{$\sim$70\%}  & \textbf{99.66$\pm$5.9} & 75.62$\pm$50.02 &  44.75$\pm$3.46 & 69.73$\pm$5.99 & 20.49$\pm$3.15 & 43.59$\pm$2.56 & 44.46$\pm$13.59 \\
 & \texttt{$\sim$20\%} & \textbf{102.85$\pm$2.26} & 19.11$\pm$24.08 & 11.94$\pm$0.88  & 19.66$\pm$3.69 & 12.37$\pm$2.96 & 20.1$\pm$2.17 & \\ \hline 
 & average & \textbf{103.83$\pm$4.48} & 67.08$\pm$43.83 & 36.75$\pm$4.7 & 67.36$\pm$4.06 & 30.27$\pm$4.93 & 46.61$\pm$2.67 & 44.46$\pm$13.59 \\ \hline 
\texttt{locomotion-} & \texttt{$\sim$110\%}  & \textbf{109.17$\pm$0.16} &  93.76$\pm$7.87 & 80.3$\pm$14.74 & 86.93$\pm$4.85 & 70.58$\pm$9.98 & 61.64$\pm$11.36 &  \\
\texttt{hopper} &\texttt{$\sim$40\%} & \textbf{108.42$\pm$0.62} & 103.9$\pm$10.28 &  40.66$\pm$3.35 & 42.65$\pm$2.86 & 38.7$\pm$3.7 & 19.63$\pm$2.3 & 64.77$\pm$10.23 \\
 & \texttt{$\sim$15\%}  & \textbf{108.01$\pm$0.64} & 75.12$\pm$28.95  &  25.2$\pm$3.58 & 24.37$\pm$2.26 & 19.54$\pm$2.14 & 10.29$\pm$1.24 & \\ \hline 
& average & \textbf{108.53$\pm$0.47} & 90.93$\pm$15.7 &  48.72$\pm$7.22 & 51.32$\pm$3.32 & 42.94$\pm$5.27 & 30.46$\pm$4.97 & 64.77$\pm$10.23 \\ 
\end{tabular}
% \end{adjustwidth}
}
\vspace{-0.2cm}
\caption{A comparison of RLIF, HG-DAgger, DAgger, and BC on continuous control tasks. RLIF consistently performs better than HG-DAgger and DAgger baselines for each individual expert level as well as averaged over all expert levels.} 
%%SL.9.28: bold the best results and add a more informative caption (see comment from 1/25 below, which says the same thing!)
\label{tab:performance}
%%SL.1.25: add a sentence of discussion about what the reader should look for in this table
\vspace{-0.6cm}
\end{center}
}
\end{table*}

The experts and $Q^{\piref}$ associated with intervention strategies are obtained by training a near-optimal policy and then randomly substituting its actions for random actions and intervention decisions to induce the desired level of suboptimality. Further details on how we train the starting policies and intervention experts can be found in  Appendix.~\ref{subsec:appen_exp_setup}. 


% \usepackage[top=0.1in, margin=1in]{geometry}





%%SL.9.28: link to anonymous website with video for the robot results
\paragraph{Results and discussion.} We report our main results in Table.~\ref{tab:performance}, with additional learning curves for analyzing learning progress in terms of the number of iterations presented in Appendix.~\ref{subsec:appen_exp_plots} and an IQL baseline in Appendix.~\ref{subsec:baseline}. 
Each table depicts different expert performance levels on different tasks (rows), and different methods with different intervention strategies (columns). Note the ``expert level'' in the table indicates the suboptimality of the expert; for example, a ``90\%'' expert means it can achieve 90\% of the reference optimal expert score of a particular task; and this score is normalized across environments as 100.0. For the remaining of the table, we report the performance of different methods w.r.t. this normalized reference score.
To start the learning process, we initialize the replay buffer with a small number of samples from a 50\% expert for all methods. We also train a BC baseline on this data to verify that it is insufficient by itself to solve the task. 
We compare RLIF with DAgger and HG-DAgger under different intervention modes and expert levels. Specifically, we run DAgger under two intervention modes: 1) the expert issues an intervention if the difference between the agent's action and the expert's action is larger than a threshold as used in~\cite{Kelly2018HGDAgger, ross2011reduction}, 2) the expert issues random intervention uniformly with a given probability across an episode.  
The results suggest several takeaways: (1) We see that regardless of the suboptimality of the experts, RLIF with value-based interventions can indeed reach good performance, even if the suboptimality gap is \emph{very large}, such as improving a 15\% expert to a score over 100.0 in the 2D-walker task. (2) RLIF with a value-based simulated interventions outperforms RLIF with random interventions, especially when the suboptimality is large; this confirms that the interventions carry a meaningful signal about the task, providing implicit rewards to RLIF. We also observe that the value-based intervention rate goes down as the agent improves itself as shown in Fig.~\ref{fig:rlif_train}, this confirms our proposed intervention model does carry useful information about the task, and works reasonably as the agent learns.
(3) RLIF outperforms both DAgger and HG-DAgger consistently across all tasks, and the performance gap is more pronounced when the expert is \emph{more suboptimal}, and can be as large as \textbf{5x}; crucially, this resonates with our motivation: the performance of DAgger-like algorithms will be subject to the suboptimality of the experts, while our method can reach good performance even with suboptimal experts by learning from the expert's decision of \emph{when} to intervene. 

% \begin{wrapfigure}{r}{0.4\textwidth}
%     \centering
%     \vspace{-0.4cm}
%      \includegraphics[width=0.4\textwidth]{figs/rlif.png} 
%     % \vspace{-0.5em}
%     \caption{RLIF results on the real-world robotic manipulation task.}
%     \label{fig:robot}
%     \vspace{-1cm}
% \end{wrapfigure}

\begin{wrapfigure}{r}{0.65\textwidth}
    \centering
     \includegraphics[width=0.65\textwidth]{figs/rlif_robot.png}
    % \vspace{-0.5em}
    \caption{\changed{RLIF results on the real-world robotic manipulation task.}}
    \vspace{-1.0em}
    \label{fig:robot}
\end{wrapfigure}

\paragraph{Ablations on Intervention Modes.} As stated in Sec.~\ref{subsec:intervention_mode}, the performance of RLIF critically depends on when the expert chooses to intervene. Now we analyze the effect of different $Q^{\piref}$ value functions on the final performance of RLIF.  We report the numbers in Table.~\ref{tab:ablation-performance} of Appendix.~\ref{subsec:ablation}. We can observe that the particular choice of $Q^{\piref}$ does heavily influence our algorithm's performance: as the $\piref$ deteriorates, $Q^{\piref}$ becomes increasingly inaccurate; thus making the intervention decision more ``uncalibrated'', which in the end translates to worse policy performance.



\subsection{Real-World Vision-Based Robotic Manipulation Task}\label{subsec:robot_task}

While we've shown that RLIF works well under reasonable models of the expert's intervention strategy, to confirm that this model actually reflects real human interventions, we next conduct an expert where a human operator supplies the interventions directly for real-world robotic manipulation tasks. \changed{The first task, shown in Fig.~\ref{fig:human}, involves controlling a 7-DoF robot arm to fit a peg into its matching shape with a very tight tolerance (1.5mm), directly from image observations. This task is difficult because it involves dealing with discontinuous and non-differentiable contact dynamics, complex high-dimensional inputs from the camera, and an imperfect human operator. The second task involves controlling the same robot arm to unfold a piece of cloth by hooking onto it and pulling it open. This task is difficult because along with also being a complex continuous control problem like the first task, it also involves manipulation of deformable objects. This task is fitting to study RLIF since it is difficult to specify rewards which makes it hard to apply regular RL. } In our setup, the human provides interventions by using a Space Mouse: whenever the human touches the Space Mouse, they will take over the control of the robot through the Space Mouse, and the human can return the control to the RL agent by disengaging with the Space Mouse. We mark the transition of the previous time step of such an intervention as a negative reward. We use an ImageNet pre-trained EfficientNet-B3~\citep{efficientnet} as a vision backbone for faster policy training. Two cameras mounted on the robot end-effector provide continuous visual feedback. More details on the setup can be found in Appendix.~\ref{subsec:appen_robot}.
\changed{We report the results in Fig.~\ref{fig:robot}. Our method can solve the insertion task with a 100\% success rate within six rounds of interactions, which corresponds to 20 minutes in wall-clock time, including robot resets, computation, and all intended stops, and the unfolding task with a 95\% success rate in seven rounds of interaction.} This highlights the practical usability of our method in challenging real-world robotic tasks. We refer the training and evaluation videos of the robotic tasks to our website: \url{rlifpaper.github.io}.

==> sections/marked_changes/method.tex <==
\section{Interactive Imitation Learning as Reinforcement Learning}\label{sec:method}

\setlength{\intextsep}{6pt}
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-1em}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
\caption{RLIF}\label{alg:rlif}
%%SL.5.17: nitpick -- in RL we need to add transitions to the dataset, not (s,a) pairs, so it should be (s,a,s')
\begin{algorithmic}[1] % The number tells where the line numbering should start
\REQUIRE $\pi$, $\piexp$, $D$
\FOR{\texttt{trial} $i = 1$ to $N$}
    \STATE Train $\pi$ on D via {\color[HTML]{B85450} reinforcement learning.}
    \FOR{\texttt{timestep} $t=1$ to $T$}
        \IF{$\piexp$ intervenes at $t$} 
            \STATE {\color[HTML]{B85450}  label $(s_{t-1},a_{t-1}, s_{t})$ with -1 reward}, \\ append to $D_i$
        \ELSE 
            \STATE {\color[HTML]{B85450} label $(s_{t-1},a_{t-1}, s_{t})$ with 0 reward}, \\ append to $D_i$
        \ENDIF
    \ENDFOR
    \STATE $D \leftarrow D \cup D_i$
\ENDFOR
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{wrapfigure}

The key observation of this paper is that, under typical interactive imitation learning settings, the \emph{intervention signal alone} can provide useful information for RL to optimize against, without assuming that the expert demonstrator actually provides optimal actions.
%In this section, we describe our practical algorithm, which we then analyze theoretically in Sec.~\ref{sec:theory} under a specific assumption about when the expert chooses to intervene, followed by an experimental evaluation where we also study a variety of different expert intervention models.
%In this section, we establish our practical algorithm  that combines the best of both worlds: the comparatively more accessible assumptions of interactive imitation learning and the capacity to improve beyond the observed performance in the data provided by RL. In Sec.~\ref{sec:theory}, we will provide theoretical analysis of our algorithm showing that it is provably better than DAgger under certain assumptions. The rest of this section is organized as follows: in Sec.~\ref{subsec:iil} we first sketch HG-DAgger, a particular on-policy variant of DAgger, which we run our method under similar settings; we then describe our algorithm in sec.~\ref{subsec:rlif} which only requires minimal changes from the mentioned HG-DAgger algorithm; finally, we explain three different intervention modes in Sec.~\ref{subsec:intervention_mode} that are used to label rewards for our method.
%%SL.5.16: Maybe phrase as something like: in Section XX, we will provide theoretical analysis of our algorithm showing that it [does something good]
%%SL.5.16: I don't really understand the point of this subsection. Is the goal just to define BC? If so, let's do this in the preliminaries, this just seems like background stuff that shouldn't be here. I suggest skipping this and getting straight to the point (and remove the 1/2 stuff above)
%\subsection{RL}\label{subsec:rlif}
% Concretely, we refer to \jlnote{Add a wrap algorithm box for DAGGER} for a general recipe for such algorithms: it alternates between training a new policy with the aggregated dataset and generating such datasets by executing the current policy with expert intervention. As previously noted, the asymptotic performance of $\pi_{\theta}$ will depend on the optimality of $\piexp$.
%%SL.5.16: Here I think we just have too much motivation. We've already spent a bunch of time motivating the idea in the intro and problem statement, let's actually explain what the method is, possibly with a diagram, pseudocode, and a clear method description
%\paragraph{Reinforcement learning for intervention minimization.}
%\label{subsec:RLIF}

Our method, which we refer to as RLIF (reinforcement learning from intervention feedback), follows a similar outline as the HG-DAgger method in Algorithm~\ref{alg:hg-dagger}, but using reinforcement learning in place of supervised learning. The generic form of our method is provided in Algorithm~\ref{alg:rlif}. On Line 2, the policy is trained on the aggregated dataset $D$ using RL, with rewards derived from interventions. The reward is simply set to 0 for any transition where the expert does not intervene, and -1 for the previous transition where an expert intervenes. After an intervention, the expert can also optionally take over the control for a few steps; after which it will be released to the RL agent. This way, an expert can also intervene multiple times during one episode.
All transitions are added to the dataset $D$, not just those that contain the expert reward; in practice, we can optionally initialize $D$ with a small amount of offline data to warm-start the process.
An off-policy RL algorithm can utilize all of the data and can make use of the reward labels to avoid situations that cause interventions. 
This approach has a number of benefits: unlike RL, it doesn't require the true task reward to be specified, and unlike interactive imitation learning, it does not require the expert interventions to contain optimal actions, though it does require the \emph{choice} of when to intervene to correlate with the suboptimality of the policy (as we will discuss later). 
Intuitively, we expect it to be less of a burden for experts to \textit{only} point out which states are undesirable rather than actually \textit{act optimally} in those states.

%As motivated in Sec.~\ref{sec:intro}, even $\piexp$ is not optimal and in the absence of true task reward; we can alternatively use RL to minimize the occurrence of expert intervention events as a means to avoid undesirable states. This has several benefits: 1) this method doesn't require true task reward to run RL which sometimes can be simply unavailable or error-prone, 2) it can improve upon suboptimal $\piexp$ where interactive imitation learning methods can't. Intuitively, it would be much less of a burden for experts to \textit{only} point out which states are undesirable rather than actually \textit{act optimally} in those states. RL algorithm is supposed to then find patterns given enough of such signals so as to ``robustify” the suboptimal expert. More rigorously, in Lemma~\ref{lemma:naive-upper-bound-main} and Theorem~\ref{thm:upperbound-mixing-ratio-main}, we prove RL under this setting can indeed converge to a $\epsilon$-optimal policy with sample complexity $\wt{O}\paren{\frac{H^3S^2\Delta}{\eps^2}}$ that depends both on the suboptimality of expert and modes of intervention; we refer to Sec.~\ref{sec:theory} for detailed theoretical discussion.

%Specifically, consider an episode $\tau = \{s_1, a_1, s_2, a_2 ... s_T, a_T\}$ by executing current policy $\pi$, where $T$ is the episode length. An expert $\piexp$ can choose to intervene at any time step $k, 2\leq k \leq T $ for certain reasons, we assign reward $r_{k-1}=-1$ to $(s_{k-1}, a_{k-1})$ pair because $a_{k-1}$ leads to an undesirable state $s_k$ that $\piexp$ has to intervene; and 0 reward otherwise. The optimization objective for RL is then to maximize rewards along episodes $\underset{\tau \sim \pi(\cdot)}{\mathbb{E}}[R(\tau)]$, where $R(\tau)$ is the accumulated rewards along an episode $\tau$.



%%SL.9.24: Generally, I found the indexing in this pseudocode really confusing. What's an epoch? The use of the term "epoch" in RL is generally incorrect (an epoch is one pass through the training set, which makes zero sense in online RL), and the use of k/t/N/etc is pretty confusing. For ex, why is line 4 k = t >= 2? That doesn't even seem like a well formed statement. Can we simply this a bit? Maybe outer loop at line 2 should be over trials, and then at line 4 we can remove this >= 2 thing? Then we can use t to index time steps instead of k

\paragraph{Practical implementation.} To instantiate Algorithm~\ref{alg:rlif} in a practical deep RL framework, one shall choose the RL algorithm carefully. Note that the data for RL is collected by a mixture of potential suboptimal expert actions and on-policy actions, which necessitates choosing a suitable off-policy RL algorithm that can incorporate prior data easily but can efficiently improve with further experience. While a variety of algorithms designed for online RL with offline data could be suitable~\citep{song2022hybrid,lee2022offline,nakamoto2023cal}, we adopt the recently proposed RLPD algorithm~\citep{ball2023efficient}, which has shown compelling results on sample-efficient robotic learning. RLPD is an off-policy actor-critic reinforcement learning algorithm that builds on soft-actor critic~\citep{sac}, but makes some key modifications to satisfy the desiderata above such as a high update-to-data ratio, layer-norm regularization during training, and using ensembles of value functions, which make it more suitable for incorporating offline data into online RL. For further details on this method, we refer readers to prior work~\citep{ball2023efficient}, though we emphasize that our method is generic and in principle could be implemented relatively easily on top of a variety of RL algorithms. The RL algorithm itself is not actually modified, and our method can be viewed as a meta-algorithm that simply changes the dataset on which the RL algorithm operates.

%%SL.9.24: This paragraph is out of date, right?

%We now discuss how to devise a practical algorithm based on the discussion so far. With reward labels coming from different intervention strategies in Sec.~\ref{subsec:intervention_mode}, our method \ours can be run under the same setting as in Alg. \jlnote{ref to the Dagger algo box} with minimum changes; on line \jlnote{refer to algo box}, swapping a supervised learning training objective with any off-the-shelf RL method to update $\pi$. Our method can in principle work with any type of RL algorithm, we choose Implict Q-learning(IQL)~\cite{kostrikov2021offlineb} because it's easy to use and particularly well-suited in our batched setting. We briefly sketch IQL algorithm here, we refer readers to~\cite{kostrikov2021offlineb} for further details. 
%\jlnote{add IQL udpate equations here. Or, actually, do we need that at all?}

==> sections/marked_changes/theory.tex <==
\section{Theoretical Analysis}\label{sec:theory}
In this section, we provide a theoretical analysis of \ours{} in terms of the suboptimality gap. We introduce our theoretical settings and goals in Sec.~\ref{subsec:assumptions}. Then we will quantify the suboptimality gap in Sec.~\ref{subsec:main-results}.

\subsection{Theoretical Settings and Assumptions}
\label{subsec:assumptions}
We consider the setting where we {\em cannot access to the true task reward} $r$, and we can only obtain rewards $\rtilde$ through interventions. For simplicity of analysis, we define this reward function as $\rtilde=\indicator{\text{Not intervened}}$ (i.e., 1 for each step when an intervention does \emph{not} happen), which differs from the reward in Algorithm~\ref{alg:rlif} by a constant and thus does not change the result, but allows us to keep rewards in the range $[0,1]$. We aim to apply RL using the intervention reward $\rtilde$ induced by \ours{}, and quantify the suboptimality gap with respect to the true reward $r$. In particular, let $\pitilde$ denote the policy learned by \ours{} for maximizing the overall return on reward function $\rtilde$: 
\begin{equation}
    \label{eq:pitilde-property}
    \pitilde\in\Pioptdelta, \text{ s.t. }  \Pioptdelta: = \arg\max_{\pi\in\Pi} \bb E_{a_t\sim \pi(s_t),\rtilde(s_t,\pi(s_t))}\brac{\sum_{t=0}^\infty\gamma^t \rtilde(s_t,a_t)|s_0\sim\mu}.    
\end{equation}
{\em Our goal is to bound the the suboptimality gap}: $\subopt:=V^{\star}(\mu) - V^{\pitilde}(\mu)$. Based on the intervention strategy specified in Eqn.~\ref{eq:soft-rational-intervention}, we introduce our definitions of $\rtilde$ as follows. 
And we'll leave the discussion of the property of the function space $\Pioptdelta$ to Appendix~\ref{sec:appendix:piopt-delta-property}.


\begin{assumption}
\label{assump:rlif-reward-def}
\changed{
For a policy $\pi\in \Pi$, the reward function $\rtilde$ induced by Alg.~\ref{alg:rlif} is defined as $\rtilde=\indicator{\text{Not intervened}}$. The probability of intervention is similarly defined as Eqn.~\ref{eq:soft-rational-intervention}, for a constant $\beta>0.5$. We assume the expert may refer to a reference policy $\piref\in \Pioptdelta$ for determining intervention strategies as mentioned in Sec.~\ref{subsec:intervention_mode}. In addition, we assume the expert's own policy will not be intervened $\piexp\in \Pioptdelta$}.\end{assumption}
%%SL.9.28: This seems to be simultaneously defining the reward (which is unnecessary as it was already defined above) and defining the intervention (which is fine, but then don't call it a reward assumption)
%%SZ.9.28: Fixed 
%Intuitively, Assumption~\ref{assump:rlif-reward-def} suggests that the expert may have some mental model of $\piref$ (via $V^{\piref}$) for {\em determining whether the agent is making a bad action}, and the expert {\em will execute $\piexp$ to override these actions}. 
%The expert has two policies: $\piexp$, which is the policy they follow when selecting \emph{actions} for intervention, and $\piref$, which is the expert's belief about the optimal policy that they will use to determine \emph{when} to intervene. 
%Note that $\piref$ might be better than $\piexp$, which means that the expert can \emph{recognize} good (or bad) behavior better than they can execute it. This is not uncommon in the case where a person might be better able to tell that the robot is doing something good or bad, but less proficient at actually controlling it to perform a better behavior.
%%SL.9.28: I don't understand what the above sentence means, it is not grammatically correct. Also, can you make sure to clearly define \piref and \piexp? I think what you want to say (perhaps in the previous definition that is currently marked incorrectly as "Reward Assumption") is something like: The expert has two policies: $\piexp(a|s)$, which is the policy they follow when selecting \emph{actions} for intervention, and $\piref(a|s)$, which is the expert's belief about the optimal policy that they will use to determine \emph{when} to intervene. Note that $\piref(a|s)$ might be better than $\piexp(a|s)$, which means that the expert can \emph{recognize} good (or bad) behavior better than they can execute it. This is not uncommon in the case where a person might be better able to tell that the robot is doing something good or bad, but less proficient at actually controlling it to perform a better behavior.
%%SZ.9.28: I removed the previous, sentence, it was not an inaccurate writing. I have merged your wording into the writing.
The $\delta$ that appears in $\rtilde$ for determining the intervention condition is similarly defined in Eqn.~\ref{eq:soft-rational-intervention} could be referred as the ``confidence level'' of the expert.
%%SL.9.28: I don't think the analogy to the "cost-to-go" term really makes sense, I would cut this part and keep it as confidence level. Note however that, as faras I can tell, the intervention model has not actually been defined yet! This is crucial to define, otherwise people will have no idea what delta means
%%SZ.9.28: I think it is defined in eqn 5.1?
Note that Assumption~\ref{assump:rlif-reward-def} is a {\em generalized} version of the DAgger, as in the DAgger case one can treat $\piref=\piexp$.
%%SL.9.28: those are two different statements, unknown or piref = piexp -- which is it?
%%SZ.9.28: Fixed

% More importantly, the reference policy $\piref$ and the expert policy $\piexp$ could be different.
%%SL.9.28: if you use my phrasing above, you don't need to restate this again
%%SZ.9.28: fixed
%Note that Assumption~\ref{assump:rlif-reward-def} is also well corroborated by our experiments in Sec.~\ref{sec:experiments}. As discussed in Sec.~\ref{sec:experiments}, we first show that one can improve the empirical performance in simulation with limited access to $Q^{\piref}$. Next, as we have also shown in human experiments, such a reference $\piref$ may come from the mental model of a human and $\piexp$ can be viewed as the human's policy. 
%%SL.9.28: what do you mean "chosen"? this is part of the person's model, you don't choose it; are you just saying you assume it's greater than 0.5? if so just say that
%%SZ:fixed
%which also corroborates with our experimental setting (Sec.~\ref{sec:experiments}) of $\beta = 0.95$.

% After an intervention, the rollout follows the (potentially suboptimal) expert policy $\piexp$, which we can formalize as the following assumption:
% \begin{assumption}
%     \label{assump:rlif-piexp}
%     We assume that we can sample from $d_\mu^{\piexp}$,
%     %%SL.9.28: what do you mean "we assume access"? we don't get access to this, we get samples, and not from this distribution, but the mixture policy with the intervention (which is not the same!)
%     %%SZ.9.28: fixed
%     the visitation distribution of $\piexp$. We will use
%     \begin{equation}
%     \label{eq:l1-norm-diff}    
%         \Deltaexp := \norm{\dpistar_\mu-\dpiexp_\mu}{1},\qquad \Deltaref := \norm{\dpistar_\mu-\dpiref_\mu}{1},
%     \end{equation}
%     to denote the difference between (1) $\piexp$ and (2) $\pistar$ and $\piref$, in terms of the $\ell^1$ norm of their state occupancy distributions.
% \end{assumption}
\changed{assumption 2 moved to appendix}

\subsection{Main Results}
\label{subsec:main-results}

% We first introduce some auxiliary definitions and preliminary results on the functional class $\Pioptdelta$ to assist the presentation of our main results. 
% \begin{definition}
%     \label{def:d_delta}
%     For the function class $\Pioptdelta$ defined in Eqn.~\ref{eq:pitilde-property}, we define a mapping ${d_{\delta}:\Pioptdelta\times \Pioptdelta\to \bb R}$ as $d_{\delta}(\pi,\pi') = \max_{s\in \mc S} \norm{\pi(\cdot|s) - \pi'(\cdot|s)}{1}$.
% \end{definition}
% A notable observation is that, Def.~\ref{def:d_delta} defines a metric over the functional space $\Pioptdelta$. 
% \begin{lemma}[Properties of $\Pioptdelta$]
% \label{lemma:d-properties-main}
% $\forall \delta >0$, $d_\delta$ is a metric over $\Pioptdelta$. Let 
% \begin{equation}
%     \label{eq:abs-pioptdelta-def}
%     \abs{\Pioptdelta}:=\max_{\pi,\pi'\in \Pioptdelta} d_\delta(\pi,\pi'),
% \end{equation}
% then $\abs{\Pioptdelta}$ is monotonic decreasing in $\delta$.
% \end{lemma}

% Lemma~\ref{lemma:d-properties-main} first introduces $d_\delta$ as a metric defined on the function space $\Pioptdelta$, and shows that the monotonic decreasing property of $\abs{\Pioptdelta}$, the maximum distance between any two policies in $\Pioptdelta$. With the monotonic decreasing property of $\abs{\Pioptdelta}$.
To provide a comparable suboptimality gap with DAgger~\citep{ross2011reduction}, we introduce the similar behavior cloning loss on $\piexp$.
\begin{definition}[Behavior Cloning Loss~\citep{ross2011reduction}]
\label{def:BC-loss}
We use the following notation to denote the 0-1 loss on behavior cloning loss w.r.t. $\piexp$ and $\piref$ as: $\ell(s,\pi(s))=\indicator{\pi(s)\neq\piexp(s)},\forall s\in \mc S$, $\ell'(s,\pi(s))=\indicator{\pi(s)\neq\piref(s)},\forall s\in \mc S$.
\end{definition}
With Assumption~\ref{assump:rlif-reward-def}, and Def.~\ref{def:BC-loss}, we now introduce the suboptimality gap of \ours{}.

\begin{theorem}[Suboptimality Gap of \ours{}]
    \label{thm:subopt-gap-main}
    Let $\pitilde\in\Pioptdelta$ denote an optimal policy from maximizing the reward function $\rtilde$ generated by \ours{}. Let ${\eps = \max\Brac{\bb E_{s\sim d_\mu^{\pitilde}}\ell(s,\pi(s)),\bb E_{s\sim d_\mu^{\pitilde}}\ell'(s,\pi(s))}}$ (Def.~\ref{def:BC-loss}). Under Assumption~\ref{assump:rlif-reward-def}, when $V^{\piref}$ is known, the \ours{} suboptimality gap satisfies:
    \changed{\begin{equation*}
        \subopt_\mr{\ours{}} = V^{\star}(\mu) - V^{\pitilde}(\mu) \leq\min\Brac{V^{\pistar}(\mu) - V^{\piref}(\mu),V^{\pistar}(\mu) - V^{\piexp}(\mu)}+\frac{\delta\eps}{1-\gamma}.
    \end{equation*}}
\end{theorem}
Note that our Assumption~\ref{assump:rlif-reward-def} is a generalized version of DAgger with the additional $V^{\piref}$, we can use the same analysis framework of Thm.~\ref{thm:subopt-gap-main} to obtain a suboptimality gap of DAgger and obtain the following suboptimality gap. 
%%SL.9.28: it's not obvious why this is true, because DAgger trains with SL, not with RL; perhaps there is a good explanation of this, but then this explanation should be added somewhere
%%SZ.9.28: added discussion
Using a similar proof strategy to Thm.~\ref{thm:subopt-gap-main}, we provide a suboptimality gap for DAgger as follows.

\changed{\begin{corollary}[Suboptimality Gap of DAgger]    
    \label{cor:subopt-gap-dagger-main}
     Let $\pitilde\in\Pioptdelta$ denote an optimal policy from maximizing the reward function $\rtilde$ generated by \ours{}. Let $\eps = \bb E_{s\sim d_\mu^{\pitilde}}\ell(s,\pi(s))$ (Def.~\ref{def:BC-loss}). Under Assumption~\ref{assump:rlif-reward-def}, when $V^{\piref}$ is unknown, the DAgger suboptimality gap satisfies:
    \begin{equation}
        \subopt_\mr{DAgger} = V^{\star}(\mu) - V^{\pitilde}(\mu) \leq V^{\pistar}(\mu) - V^{\piexp}(\mu)+ \frac{\delta\eps}{1-\gamma}.
    \end{equation}
\end{corollary}}

\changed{A direct implication of Thm.~\ref{thm:subopt-gap-main} and Cor.~\ref{cor:subopt-gap-dagger-main} is that, under Assumption~\ref{assump:rlif-reward-def}, \ours{} is at least as good as DAgger, since $\subopt_\mr{\ours{}}\leq\subopt_\mr{DAgger}$. We will provide a bandit example below to show that our upper bounds in Thm.~\ref{thm:subopt-gap-main} and Cor.~\ref{cor:subopt-gap-dagger-main} are tight.
\begin{example}[Lower Bounds]
\label{exp:tight-rlif-bound}
    Consider a bandit problem where we have only one state $\mc S =\{s\}$, two actions $\mc A = \{a_1,a_2\}$ and, and the reward function is given as $r(a_1) = 1$ and $r(a_2) = 0$. Assume the policy space $ \Pi\subset\bb R^2_+$ is a two-dimensional Euclidean space, where each policy $\pi\in\Pi$ satisfies such that $\pi(a_1)+\pi(a_2)=1$. Let $\piref,\piexp\in \Pi$ be any two policies in the policy space, and $\pitilde\in\Pioptdelta$ be the optimal policy from maximizing the reward function $\rtilde$ generated by \ours{}, ${\eps = \max\Brac{\bb E_{s\sim d_\mu^{\pitilde}}\ell(s,\pi(s)),\bb E_{s\sim d_\mu^{\pitilde}}\ell'(s,\pi(s))}}$ (Def.~\ref{def:BC-loss}). Then we have
    \begin{align*}
        \subopt_\mr{\ours{}}
        = &\;\min\Brac{V^{\pistar}(\mu) - V^{\piref}(\mu),V^{\pistar}(\mu) - V^{\piexp}(\mu)}+\frac{\delta\eps}{1-\gamma},\\
        \subopt_\mr{DAgger}
        = &\;V^{\pistar}(\mu) - V^{\piexp}(\mu)+\frac{\delta\eps}{1-\gamma}.
    \end{align*}
\end{example}}


\changed{We leave the proof of Thm.~\ref{thm:subopt-gap-main}, Cor.~\ref{cor:subopt-gap-dagger-main} and Exp.~\ref{exp:tight-rlif-bound} analysis under our framework to Appendix~\ref{sec:appendix:subopt-gap-inf-sample}. For completeness, we also provide a non-asymptotic sample complexity analysis for learning an $\pihat$ that maximizes $V^\pi_{\rtilde}(\mu)$ in Appendix~\ref{sec:appendix:non-asy-bound}. Our non-asymptotic result in Cor.~\ref{coro:sample-complexity-offline} suggests that the total sample complexity {\em does not exceed} the sample complexity $\wt{O}\paren{\frac{SC^\star_\mr{exp}}{(1-\gamma)^3\eps^2}}$, where $C^\star_\mr{exp}$ is the concentrability coefficient w.r.t. $\piexp$ (formally defined in Def.~\ref{def:concen-coeff}). }





==> sections/misc.tex <==
\section{Additional Theoretical Results}\label{sec:appendix-thy}

\subsection{Human Expert Intervention}
\label{subsec:appendix:intervention}

\begin{theorem}[Concentrablity of a Intervention Probability, Thm.~\ref{thm:upperbound-mixing-ratio-main} restated]
    \label{thm:upperbound-mixing-ratio}
    Suppose the Assumption~\ref{assump:confidence-subset} hold. In addition, if we construct $\muint$ by mixing $\dpiexp$ with probability $\beta$ ($0<\beta<1$) and a uniform distribution over $\smcbar$:
    \begin{equation}
        \label{eq:muint-def-appendix}
        \muint_{h} = (1-\beta) \unif\paren{\smcbar} + \beta \dpiexp_h,\quad \forall h\in[H],
    \end{equation}
    then the concentrability coefficient satisfies $C^\star_{\muint}\leq f(\beta):= \frac{\sbar\Delta}{1-\beta}+\frac{1}{\beta}$, where $\Delta$ is defined in Eqn.~\ref{eq:l1-norm-diff-exp}.
    Furthermore, we also have $\min_{\beta}f(\beta) = \sbar \Delta+2\sqrt{\sbar \Delta}+1$, which can be achieved by setting the intervention probability $\beta = \frac{1}{1+\sqrt{\sbar\Delta}}$. 
\end{theorem}

\begin{proof}
\label{proof:upperbound-mixing-ratio}
Notice that the optimal policy $\pistar$ is a deterministic policy, we have $d_h^{\pistar}(s,a) = d_h^{\pistar}(s)\indicator{\pistar(s)=a}$. Hence, applying the similar decomposition technique shown in~\cite{li2023understanding}, we have
\begin{equation}
    \begin{split}
        &\;\max_{s,a} \frac{\dpistar_h(s,a)}{\muint_h(s,a)}=\norm{\frac{\dpistar_h}{\muint_h}}{\infty} \leq \norm{\frac{\dpistar_h-\dpiexp_h}{\muint_h}}{\infty} + \norm{\frac{\dpiexp_h}{\muint_h}}{\infty}\\
        =&\; \norm{\frac{\dpistar_h-\dpiexp_h}{(1-\beta) \unif\paren{\sbar} + \beta \dpiexp_h}}{\infty} + \norm{\frac{\dpiexp_h}{(1-\beta) \unif\paren{\sbar} + \beta \dpiexp_h}}{\infty}\\
        \leq&\; \norm{\frac{\dpistar_h-\dpiexp_h}{(1-\beta) \unif\paren{\sbar}}}{\infty}+ \norm{\frac{\dpiexp}{\beta\dpiexp}}{\infty}\leq  \frac{\sbar\norm{\dpistar_h-\dpiexp_h}{1}}{1-\beta}+\frac{1}{\beta}\leq\frac{\smcbar\Delta}{1-\beta}+\frac{1}{\beta}.
    \end{split}
\end{equation}
Note that the above inequality holds $\forall h\in[H]$, hence, we conclude that 
\begin{equation}
    C_{\muint}^\star = \max_{s,a,h} \frac{\dpistar_h(s,a)}{\muint_h(s,a)}\leq \frac{\sbar\Delta}{1-\beta}+\frac{1}{\beta}.
\end{equation}
If we further view $f(\beta)=\frac{\sbar\Delta}{\beta}+\frac{1}{1-\beta}$ as a function of beta, by setting $\beta$ such that $f'(\beta) = 0$, we obtain
\begin{equation}
    f_{\min}(\beta) = f\paren{\frac{1}{1+\sqrt{\sbar \Delta}}} = \sbar \Delta+2\sqrt{\sbar \Delta}+1,
\end{equation}
which completes the proof.
\end{proof}



\subsection{Extension to Stochastic Rewards}
\sz{need to move the section to experiments so that it matches the true reward}
Note that our sample complexity results of RL in Section~\ref{subsec:appendix:intervention} (or equivalently Section~\ref{sec:theory} in the main text) can be easily extended to the stochastic reward functions that are more closely related to the rational intervention strategy described in Eqn.~\ref{eq:rational-intervention}:
\begin{equation}
    \label{eq:intervention-reward-rand}
     \begin{cases}
        r_h(s,a) \sim\mr{Ber}(\beta), &  \text{if } a=\pi^\star(s),\\
        r_h(s,a) \sim\mr{Ber}(1-\beta), &  \text{otherwise,}
    \end{cases}
\end{equation}
where $\mr{Ber}$ is the Bernoulli random distribution. Note that the randomized reward $r_h$ specified above the exact setting following the rational intervention strategy specified in Eqn.~\ref{eq:rational-intervention}, as the agent only receives reward from expert interventions, and the expert intervenes with probability $\beta$ when $a\neq \pi^\star(s)$.

Since in the stochastic reward case (as specified in Eqn.~\ref{eq:intervention-reward-rand}), following the expert policy $\pi^\star$ still leads to the maximum rewards when $\beta>0.5$, as we have chosen a $\beta = 0.95$ in our experiments. Hence we can still apply the convergence result in Thm.~\ref{thm:offline-rl-sota} to the concentrability coefficient specified in Thm.~\ref{thm:upperbound-mixing-ratio-main} (or equivalently Thm.~\ref{thm:upperbound-mixing-ratio}). Therefore, our regret bound of RLIF specified in Cor.~\ref{corollary:regret-ours-main} still holds in the randomized reward setting specified in Eqn.~\ref{eq:intervention-reward-rand}. 


\sz{9.24: --- Old and broken theory below, please ignore everything below ---}
%%SL.9.24: Can we start by stating the goals, and the technical assumption about suboptimality gap can come later?
Since we only obtain reward signals from expert intervention, we consider the following reward function $r$: $r_h(s,a) =\indicator{\text{Not Intervened}}$. Intuitively, the reward of interest $r$ assigns the agent a positive reward of +1 whenever the expert does not intervene.
%%SL.9.24: Very important: we need to make it clear that there is a distinction between the (unknown) task reward and the intervention reward. Our analysis of regret should be the regret of the *task* reward. It doesn't make sense to analyze regret of the intervetnion reward.

% \subsection{The Regret of \ours{}}
% \label{subsec:bounding-concentrability-coeff}

%%SL.9.24: can we provide a brief (one sentence) context for what offline RL/LCB has to do with this? it might not be obvious to many readers

As discussed in prior RL theory work~\citep{xie2021policy,li2022settling}, for learning an $\eps$-optimal policy $\pihat$ such that $\bb E_{s\sim\mu}\brac{V_1^{\pistar}(s) - V_1^{\pihat}(s)}\leq \eps$, the tight sample complexity of offline RL (in terms of the number of trajectories) is $\wt{O}\paren{\frac{H^3SC_\mu^\star}{\eps^2}}$. Notice that the concentrability coefficient $C_{\muint}^\star$ is one of the major components that affect the final sample complexity, we will discuss how \ours{} affects the upper bound of $C_{\muint}^\star$.
%%SL.9.24: This is not discussing the reward discrepancy or intervention stuff at all, unclear what the relevance of this is. Obviously the major challenge for us is *not* concentrability, it's the reward, though perhaps once we explain how resolve that challenge, talking about concentrability might make sense.

In practice, even if the human expert does not always make the optimal decision, it is rather easy for the human expert to tell which states should not be visited by the optimal policy $\pistar$, as we will demonstrate in Sec.~\ref{sec:experiments}. To elaborate on this observation, we introduce the following assumption:
\begin{assumption}[Confidence Subset]
    \label{assump:confidence-subset}
    We assume the support $\smcbar:=\supp\paren{\dpiexp}\subset{\mc S}$ of the visitation of $\piexp$ satisfies $\supp\paren{\dpistar}\subset\smcbar$.
\end{assumption}
%%SL.9.24: Can we explain intuitively what this means? I think this is saying the support of the optimal policy is inside the support of the expert policy (which is to say expert policy covers optimal policy). That's a strong assumption, but probably OK. Still need to explain this, and we should also make it clear what pi* is (i.e., optimal for the unknown reward)
We first introduce a na\"ive upper bound of the concentrability coefficient $C^\star_{\muint}$ in the following lemma.
%%SL.9.24: it's stated as a theorem, not a lemma -- was there some reorganization glitch?

%%SL.9.24: can you provdie some intuition for what this is trying to do?
\begin{theorem}[Concentrablity of a Intervention Probability]
    \label{thm:upperbound-mixing-ratio-main}
    Suppose the Assumption~\ref{assump:confidence-subset} hold. In addition, if we construct $\muint$ by mixing $\dpiexp$ with probability $\beta$ ($0<\beta<1$) and a uniform distribution over $\smcbar$:
    %%SL.9.24: what's the rationale for the uniform distribution thing?
    \begin{equation}
        \label{eq:muint-def}
        \muint_{h} = (1-\beta) \unif\paren{\smcbar} + \beta \dpiexp_h,\quad \forall h\in[H],
    \end{equation}
    then the concentrability coefficient satisfies $C^\star_{\muint}\leq f(\beta):= \frac{\sbar\Delta}{1-\beta}+\frac{1}{\beta}$, where $\Delta$ is defined in Eqn.~\ref{eq:l1-norm-diff-exp}.
    Furthermore, we also have $\min_{\beta}f(\beta) = \sbar \Delta+2\sqrt{\sbar \Delta}+1$, which can be achieved by setting the intervention probability $\beta = \frac{1}{1+\sqrt{\sbar\Delta}}$. 
\end{theorem}
The proof of~\ref{thm:upperbound-mixing-ratio-main} is deferred to Appendix~\ref{subsec:appendix:intervention}. Applying upper bound of $C_{\muint}^\star$ to the sample complexity result in~\citet{li2022settling} (stated as Thm.~\ref{thm:offline-rl-sota} in Appendix~\ref{subsec:appendix:prior-offline-rl} for completeness), we immediately obtain the following regret bound of \ours{}:
\begin{corollary}[Regret of \ours{}]
\label{corollary:regret-ours-main}
Suppose the conditions in Theorem~\ref{thm:upperbound-mixing-ratio-main} hold, with high probability, \ours{} obtains a policy $\pihat$ such that $\bb E_{s\sim\mu} \brac{V_1^{\pistar}(s)-V_1^{\pihat}(s)}\leq\eps$, with the sample complexity of $\wt{O}\paren{\frac{H^3S}{\eps^2}\paren{\frac{S\Delta}{1-\beta}+\frac{1}{\beta}}}$, which can be further reduced to $\wt{O}\paren{\frac{H^3S^2\Delta}{\eps^2}}$ by choosing $\beta = 1/(1+\sqrt{\smcbar\Delta})$.
\end{corollary}
%%SL.9.24: how does this resolve the reward discrepancy?
\paragraph{Conclusion.}
Our theoretical conclusion is that, while the suboptimality gap $\Delta$ incurs an additional regret $H\Delta$ to DAgger, Cor.~\ref{corollary:regret-ours-main} indicates that \ours{} still can obtain an $\eps$-optimal policy (at the cost of additional sample complexity). Hence, we conclude that {\em \ours{} is generally better than DAgger when the expert data $\piexp$ is suboptimal}.

\sz{--- Old theory above --- }


\subsection{Suboptimality Gap of Imitation Learning Induced by Non-Optimal Human Experts}
\label{subsec:subopt-gap}
In this subsection, we first introduce the suboptimality gap between the non-optimal human expert $\piexp$ and the optimal $\pistar$ as the $\ell^1$ norm of the state occupancy distribution:
\begin{equation}
% \label{eq:l1-norm-diff-exp}    
    \Delta := \max_{h\in[H]}\norm{d_h^{\pistar}- d_h^{\piexp}}{1}=\max_{h\in[H]}\sum_{s\in \mc S}\abs{d_h^{\pistar}(s)-d_h^{\piexp}(s)}.
\end{equation}
Then we will demonstrate that such a suboptimality gap $\Delta$ will incur an additional regret that scales linearly with the horizon $H$ in Thm.~\ref{thm:subopt-gap-main} for imitation learning with DAgger~\citep{ross2011reduction} using $\piexp$.

\begin{theorem}[Non-Optimal Human Expert Suboptimality Gap]
\label{thm:subopt-gap-main}
Suppose $\pihat$ is the policy learned by DAgger, with a non-optimal human expert actions produced by $\piexp$, then we have 
\begin{equation}
    \bb E_{s\sim\rho} \brac{V_1^{\pistar}(s)-V_1^{\pihat}(s)}\leq H\paren{\Delta+2}+\wt{\regret} \paren{\pihat},
\end{equation}
where $\dpistar,\dpiexp\in \bb R^{S}$ are vectors of the occupancy distributions with respect to $\pistar,\piexp$, $\wt{\regret}\paren{\pihat}:=\bb E_{s\sim\rho}\brac{\vtilde^{\piexp}_1(s)-\vtilde^{\pihat}_1(s)}$ is the regret between the learned policy against the non-optimal human expert policy $\piexp$, where $\vtilde^\pi$ denotes the value function w.r.t. $\pi$ under reward $\rtilde$ and $\rtilde_h(s,a):= \indicator{a=\piexp(s)}$ is the 0-1 reward defined by following $\piexp$. $\Delta$ is defined in Eqn.~\ref{eq:l1-norm-diff-exp}.
\end{theorem}

Intuitively, the linear dependency on the horizon in Thm.~\ref{thm:subopt-gap-main} matches the linear horizon regret in Dagger~\citep{ross2011reduction} as well. Next, we will introduce the regret of \ours{}.


\section{subopt main theorem}
\begin{theorem}[Non-optimal Human Expert Suboptimality Gap, Thm.~\ref{thm:subopt-gap-main} restated]
\label{thm:subopt-gap}
Suppose $\pihat$ is the learned policy of Dagger with policy $\piexp$ or RL with $\rtilde$, then we have 
\begin{equation}
    \bb E_{s\sim\rho} \brac{V_1^{\pistar}(s)-V_1^{\pihat}(s)}\leq H\paren{\Delta+2}+\wt{\regret} \paren{\pihat},
\end{equation}
where $\dpistar,\dpiexp\in \bb R^{S}$ are vectors of the occupancy distributions with respect to $\pistar,\piexp$ and $\wt{\regret}\paren{\pihat}:=\bb E_{s\sim\rho}\brac{\vtilde^{\piexp}_1(s)-\vtilde^{\pihat}_1(s)}$ is the regret between the learned policy against the non-optimal human expert policy $\piexp$, and $\Delta$ is defined in Def.~\ref{eq:l1-norm-diff-exp}.
\end{theorem}

\begin{proof}
\label{proof:subopt-gap}
$\forall s\in \mc S$, notice that 
\begin{equation}
    \begin{split}
        V_1^{\pistar}(s)-V_1^{\pihat}(s) =  \underbrace{V_1^{\pistar}(s)-\vtilde_1^{\piexp}(s)}_{\Gamma_1(s)}+\underbrace{\vtilde_1^{\piexp}(s)-\vtilde_1^{\pihat}(s)}_{\Gamma_2(s)}+\underbrace{\vtilde_1^{\pihat}(s)-V_1^{\pihat}(s)}_{\Gamma_3(s)},
    \end{split}
\end{equation}
we have
\begin{equation}
    \begin{split}
        &\;\bb E_{s\sim\rho} \brac{V_1^{\pistar}(s)-V_1^{\pihat}(s)} = \bb E_{s\sim\rho}\brac{\Gamma_1(s)+\Gamma_2(s)+\Gamma_3(s)}.
    \end{split}
\end{equation}
Now we will calculate $\bb E_{s\sim\rho}\brac{\Gamma_1(s)},\bb E_{s\sim\rho}\brac{\Gamma_2(s)},\bb E_{s\sim\rho}\brac{\Gamma_3(s)}$. For $\bb E_{s\sim\rho}\brac{\Gamma_1(s)}$, we have 
\begin{equation}
    \begin{split}
        &\;\bb E_{s\sim\rho} \brac{\Gamma_1(s)} = \bb E_{s\sim\rho} \brac{V_1^{\pistar}(s)-V_1^{\piexp}(s)}\\
        =&\;\sum_{h=1}^H\sum_{(s_h,a_h)}\brac{ \indicator{\pistar(s_h)=a_h}d_h^{\pistar}(s_h)-\indicator{\pistar(s_h)=a_h,\piexp(s_h)=a_h}d_h^{\piexp}(s_h)}\\
        =&\;\sum_{h=1}^H\sum_{(s_h,a_h)}\Big[ \indicator{\pistar(s_h)=a_h,\piexp(s_h)=a_h}\paren{d_h^{\pistar}(s_h)-d_h^{\piexp}(s_h)}\\
        &+\indicator{\pistar(s_h)=a_h,\piexp(s_h)\neq a_h}\dpistar_h(s_h)\Big]\\
        \leq&\; H\paren{\norm{d_h^{\pistar}-d_h^{\piexp}}{1}+1}
    \end{split}
\end{equation}
where equality $(i)$ holds by applying Lemma~\ref{lemma:reward-relation} to $V_1^{\pistar},\vtilde_1^{\piexp}$. For $\bb E_{s\sim\rho}\brac{\Gamma_2(s)}$, we have $\bb E_{s\sim\rho}\brac{\Gamma_2(s)} = \bb E_{s\sim\rho} \brac{\vtilde_1^{\piexp}(s)-\vtilde_1^{\pihat}(s)} =\wt{\regret}\paren{\pihat}$. For $\bb E_{s\sim\rho}\brac{\Gamma_3(s)}$, we have 
\begin{equation}
    \begin{split}
    &\;\bb E_{s\sim\rho} \brac{\Gamma_3(s)} = \bb E_{s\sim\rho}\brac{\vtilde_1^{\pihat}(s)-V_1^{\pihat}(s)}\\
    =&\;\sum_{h=1}^H\sum_{(s_h,a_h)}\brac{ \indicator{\piexp(s_h)=a_h,\pihat(s_h)=a_h}d_h^{\pihat}(s_h)-\indicator{\pistar(s_h)=a_h,\pihat(s_h)=a_h}d_h^{\pihat}(s_h)}\\
    \leq &\; H.
    \end{split}
\end{equation}
Sum up $\bb E_{s\sim\rho}\brac{\Gamma_1(s)+\Gamma_2(s)+\Gamma_3(s)}$, we have
\begin{equation}
    \begin{split}
    \bb E_{s\sim\rho}\brac{\Gamma_1(s)+\Gamma_2(s)+\Gamma_3(s)}\leq H\paren{\Delta+2}+\wt{\regret} \paren{\pihat}
    \end{split}
\end{equation}
which finishes the proof. 
\end{proof}


\subsection{Suboptimality Gap of Non-optimal Human Expert}
\label{subsec:appendix:subopt-gap}

\begin{lemma}[Value Function of following a Deterministic Policy]
\label{lemma:reward-relation}
For two given deterministic policies $\pi,\pitilde$, suppose the reward function $r$ of the $\mc M = \{\mc S,\mc A, H, P, r\}, \tilde{\mc M}$ is the 0-1 supervised learning reward induced by following the policy $\pi$
\begin{equation}
    r_h(s,a) = \begin{cases}1&\text{if }a = \pi(s)\\ 0&\text{otherwise} \end{cases}.
\end{equation}
Then $\bb E_{s\sim\rho}\brac{V_1^{\pitilde}(s)}$ satisfies:
\begin{equation}
     \bb E_{s\sim\rho}\brac{V_1^{\pitilde}(s)} = \sum_{h=1}^H\sum_{(s_h,a_h)\in \mc S\times \mc A} \indicator{\pitilde(s_h)=a_h}\indicator{\pi(s_h)=a_h}d_h^\pi(s_h).
\end{equation}
\end{lemma}
\begin{proof}
\label{proof:reward-relation}
By the definition of $V_h^{\pitilde}$, we know that 
    \begin{equation}
        \begin{split}
            \bb E_{s\sim\rho}\brac{\vtilde^\pi_1(s)} &= \bb E\brac{\sum_{h=1}^Hr_h(s_h,a_h)|s_1\sim\rho;\pitilde}=\sum_{h=1}^H\sum_{(s_t,a_t)\in \mc S\times \mc A} r_h(s_h,a_h)d^{\pitilde}_h(s_h,a_h)\\
            &=\sum_{h=1}^H\sum_{(s_h,a_h)\in \mc S\times \mc A} \indicator{\pi(s_h)=a_h}\indicator{\pitilde(s_h)=a_h}d_h^{\pitilde}(s_h)\\
            &=\sum_{h=1}^H\sum_{(s_h,a_h)\in \mc S\times \mc A} \indicator{\pi(s_h)=a_h,\pitilde(s_h)=a_h}d_h^{\pitilde}(s_h)
        \end{split}
    \end{equation}
    which finishes the proof.
\end{proof}


==> sections/short_discussion.tex <==
\section{Discussion and Limitations}\label{sec:discussion}
Our approach does have a number of limitations. First, we require an RL method that can actually train on all of the data collected by both the policy and the intervening expert. This is not necessarily an easy RL problem, as it combines off-policy and on-policy data. That said, we were able to use an off-the-shelf offline RL algorithm (RLPD) without modification. Second, imitation learning is often preferred precisely because it doesn't require online deployment at all, and this benefit is somewhat undermined by interactive imitation learning methods. While in practice deploying a policy under expert oversight might still be safer (e.g., with a safety driver in the case of autonomous driving), investigating the safety challenges with such online exploration is an important direction for future work. 

